Nested Bregman Iterations for Decomposition Problems

We consider the task of image reconstruction while simultaneously decomposing the reconstructed image into components with different features. A commonly used tool for this is a variational approach with an infimal convolution of appropriate functions as a regularizer. Especially for noise corrupted observations, incorporating these functionals into the classical method of Bregman iterations provides a robust method for obtaining an overall good approximation of the true image, by stopping early the iteration according to a discrepancy principle. However, crucially, the quality of the separate components depends further on the proper choice of the regularization weights associated to the infimally convoluted functionals. Here, we propose the method of Nested Bregman iterations to improve a decomposition in a structured way. This allows to transform the task of choosing the weights into the problem of stopping the iteration according to a meaningful criterion based on normalized cross-correlation. We discuss the well-definedness and the convergence behavior of the proposed method, and illustrate its strength numerically with various image decomposition tasks employing infimal convolution functionals.

==> Chapters/Numerics.tex <==
\section[Numerical results]{Numerical results\footnote{The program code is available as ancillary file from the arXiv page of this paper.}}\label{sec:numerical_results}

In all of our numerical experiments we follow the standard discretization strategy, regarding functions and their derivatives. In particular, the discrete gradient, realised by a matrix and denoted by $D$,is defined using forward finite differences. We note however that more sophisticated discretisations of the gradient and its adjoint are conceivable \cite{}. 

\subsection{$\ell^1-\ell^2$}
We consider the denoising problem $(A= Id)$ for a $1-$dimensional signal consisting of $2$ components. The first component $u^*$ is  a discretization of one period of a sine curve on $n = 300$ equidistant nodes. The second component consists of multiple peaks. The noisy observation was created by adding Gaussian noise $n^\delta$ (mean $0$ and variance $\sigma = 0.05$) to the sum of the components: $f^\delta  = u^*+v^* +n^\delta$ (see the first line in figure \ref{fig:nested_morozov_l1_l2}). We then employ Algorithm \ref{algo:NestedBregman_Noisy_Morozov} with $g = \frac{\alpha}{2}\norm{D\cdot }_2$ and $h = \norm{\cdot}_1$, where $D$ is the following matrix
%where $D$ denotes a finite difference matrix.% defined at the start of the section
\begin{equation*}
    D = \begin{pmatrix*}
        &1&-1& &0\\
        &&\ddots&\ddots&&\\
        &0&&1&-1
    \end{pmatrix*}
\end{equation*}

From the creation of the data, we know the exact noise level $\delta = \norm{n^\delta}_2$. This means in each step of the algorithm we are solving \begin{equation}\label{eq:l1_l2_numrics_functional_morozov}
    \begin{cases}
        &\min \frac{\alpha}{2} \norm{Du}_2^2 + \norm{v}_1 - p_l^\delta\cdot u,\\
        &s.t \quad \norm{u+v}_2\le \delta.
    \end{cases}
\end{equation}
For the numerical solution of this problem, we employ the \textit{CVX} package for Matlab. Since $g$ is differentiable, we can update the subgradient according to $p_l^\delta = \alpha D^{*}Du_l^\delta$.
The iterates $(u_l^\delta, v_l^\delta)$ for the choice $\alpha = 400$ can be seen in lines $2$ to $5$ of Figure \ref{fig:nested_morozov_l1_l2}. The first line shows the initial step $(l = 0)$ for the Morozov regularization \eqref{eq:l1_l2_numrics_functional_morozov} with $p_0^\delta = 0$. Lines $3$ to $5$ show the minimizing pairs after $l = 1,3,29$ iterations. In the initial step, the component $v_0^\delta$ identifies all peaks from the true component $v^*$ but also contains some smaller peaks, that are not contained in $v^*$. This is because $\alpha$ is chosen too small resulting in $v_0^\delta$ being slightly over-regularized. Within the iterations, the smaller additional peaks disappear, while the larger peaks shrink. This results in the visually best approximation in step $l=4$ (line 4 in figure \ref{fig:nested_morozov_l1_l2}). With more iterations, the component $v_l^\delta$ shrinks to $0$, which also negatively influences the quality of the other component $u_l^\delta$. This is exemplified in line 5, which corresponds to the step $l = 29$. Furthermore, we were able to numerically confirm the bound for the values $h(v_l^\delta)$. This is illustrated in Figure \ref{fig:nested_morozov_l1_l2_bound}, where the full line shows the values of $h(v_l^\delta)$ and the dotted line shows the theoretical upper-bound $\frac{\alpha\norm{D (u^*+v^*)}_2^2}{l}$ from Theorem \ref{thm:Convergence_Nested_Bregman-Morozov}. Clearly, the value $h(u_l^\delta)$ decreases significantly below the theoretical bound. This suggests a possible improvement of \eqref{eq:Convergence_h_noisy}, since we also observed this behavior in other numerical experiments as well.\\
Figure \ref{fig:nested_bregman_l1_l2} shows the same experiment with Algorithm \ref{algo:NestedBregman_Noisy} instead. We want to stress that in general, one can not simply compare Algorithm \ref{algo:NestedBregman_Noisy_Morozov} and Algorithm \ref{algo:NestedBregman_Noisy}, since their iterations depend on the parameter choice made to obtain the initial iterate. Thus, for a fair comparison, it would be necessary to compute $\alpha$ and $\beta$ such that the first minimization problem in Algorithm \ref{algo:NestedBregman_Noisy} computes the same pair of minimizers as the first minimization in \ref{algo:NestedBregman_Noisy_Morozov}. In other words,  the pair$(\alpha,\beta)$ needs to be the Lagrange multiplier of \eqref{eq:NestedBregman_Morozov_initial}.



\begin{figure}[H] 
\centering
\hspace{-1cm}\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/u_real.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/v_real.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
   \scalebox{.4}{\input{Images/Images_l1_l2/f.tex}}
\end{minipage}\hspace{2cm}


\centering
\hspace{-1cm}\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Morozov/u_1.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Morozov/v_1.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Morozov/u_1+v_1.tex}}
\end{minipage}\hspace{2cm}


\centering
\hspace{-1cm}\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Morozov/u_2.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Morozov/v_2.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Morozov/u_2+v_2}}
\end{minipage}\hspace{2cm}

\centering
\hspace{-1cm}\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Morozov/u_4}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Morozov/v_4}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Morozov/u_4+v_4}}
\end{minipage}\hspace{2cm}

\centering
\hspace{-1cm}\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/u_30}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/v_30.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/u_30+v_30}}
\end{minipage}\hspace{2cm}




\caption{First line: true components and noisy observation. Lines 2-5: reconstructed components obtained by Algorithm \ref{algo:NestedBregman_Noisy_Morozov} with $\alpha =400$ and $g,h$ as in \eqref{eq:l1_l2_numrics_functional_morozov} for the iteration steps $l = 1,2,4,30$.}

\label{fig:nested_morozov_l1_l2}

\end{figure}



\begin{figure}[H] 
\centering
\hspace{-1cm}\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/u_real.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/v_real.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
   \scalebox{.4}{\input{Images/Images_l1_l2/f.tex}}
\end{minipage}\hspace{2cm}


\centering
\hspace{-1cm}\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/u_1.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/v_1.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/u_1+v_1.tex}}
\end{minipage}\hspace{2cm}

\centering
\hspace{-1cm}\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/u_2.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/v_2.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/u_2+v_2}}
\end{minipage}\hspace{2cm}

\centering
\hspace{-1cm}\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/u_4}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/v_4}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/u_4+v_4}}
\end{minipage}\hspace{2cm}

\centering
\hspace{-1cm}\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/u_30}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/v_30.tex}}
\end{minipage}\hspace{4cm}
\begin{minipage}[c]{0.1\textwidth}
    \scalebox{.4}{\input{Images/Images_l1_l2/Images_Nested/u_30+v_30}}
\end{minipage}\hspace{2cm}
\caption{First line: true components and noisy observation. Lines 2-5: reconstructed components obtained by Algorithm \ref{algo:NestedBregman_Noisy} with $\alpha =400$, $\beta = 1$ and $g,h$ as in \eqref{eq:l1_l2_numrics_functional_morozov} for the iteration steps $l = 1,2,4,30$.}

\label{fig:nested_bregman_l1_l2}

\end{figure}

\begin{figure}[H]
    \centering
    \scalebox{.5}{\input{Images/Images_l1_l2/Comparison_Morozov_Nested}}
    \caption{Values of $h(v_l^\delta)$ in Algortihms \ref{algo:NestedBregman_Noisy_Morozov} and \ref{algo:NestedBregman_Noisy} vs the theoretical upper-bound from \eqref{eq:Convergence_h_noisy}.}
    \label{fig:nested_morozov_l1_l2_bound}
\end{figure}


\subsection{$TV-H^1$}
We revisit the example from Section \ref{sec:Deomposition_Problems}. For the ratio $\frac{\alpha}{\beta} = 0.001$, we observed that the total variation component $v$ was overrepresented in both the variational regularization and Bregman iterations. We therefore use Algorithm \ref{algo:NestedBregman_Noisy_Morozov} to decrease its share in the decomposition. Figure \ref{fig:Nested_Morozov_rat=0.001_PSNR} shows the PSNR values for each iteration and Figure \ref{fig:Nested_Morozov_ratio=0.001}, we see the reconstructions after $l = 1,8,16,50$ iterations. We observe that the PSNR value increases for the first $16$ iterations and decreases from iteration $22$ on. The best PSNR value is attained at iteration $16$, which also yields a good reconstruction of the components (Line 4 in Figure \ref{fig:Nested_Morozov_ratio=0.001}). Generally, we confirm the theoretical results as the smooth component $u$ becomes more dominant during the iteration and eventually or overrepresented (Line 5 in Figure \ref{fig:Nested_Morozov_ratio=0.001}). Running the same experiment with Algorithm \ref{algo:NestedBregman_Noisy} yields similar results and the results can be seen in Figures \ref{fig:Nested_Bregman_rat=0.001_PSNR} and \ref{fig:Nested_Bregman_ratio=0.001}. We used the parameter choice $\alpha = 465$, $\beta = 0.465$, i.e. we applied the Nested Bregman procedure to the results of line 2 in Figure \ref{fig:bregman_deblurring}. In this case, the best PSNR value was achieved after $15$ iterations. Generally, we observe that the PSNR values are slightly larger than the ones obtained with Algorithm \ref{algo:NestedBregman_Noisy_Morozov} for the same number of iterations. This is expected, as instead of solving a single minimization problem, we now have an inner loop consisting of Bregman iterations (see the discussion of Bregman iterations in section \ref{sec:Deomposition_Problems}). We conclude that in both experiments, the Nested Bregman iterations can significantly improve the quality of the decomposition, which consequently also increases the PSNR of the overall reconstruction. 


\kp{todo: comparing Figures 1 and to Figures 4,5, i.e. what are the advantages of Alg 2,3 over the traditional variational approaches: In the latter we do have to search for two parameters "manually", and look visually for the best decomposition. We end up solving the problems many times with a big computational burden. With Alg 2,3 on the other hand, we do not put too much effort on the choice of alpha and beta, - some reasonable initialisation is enough. We run the iteration and the only choice we have to make is where to stop (again visually. The overall computational time is lower (need to provide some indicative runnning times). Some comments on the larger plateau of Figure \ref{fig:nested_morozov_l1_l2_bound} (maybe have an analogous figure here as well) + we get larger PSNR}

\begin{figure}[H]
    \centering
    \includegraphics[scale = 0.5]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/PSNR.png}
    \caption{PSNR values for the iterates obtained by Algorithm \ref{algo:NestedBregman_Noisy_Morozov}  with $g(u) = \frac{1}{2}\norm{\nabla u}_{L^2}^2 $ and $ \beta h(v)=  \beta\tv{v}$ for initial choice $\beta = \frac{1}{0.001}$.}
    \label{fig:Nested_Morozov_rat=0.001_PSNR}
\end{figure}

\begin{figure}[H]
\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/data/u.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/data/v.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/data/u+v.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/data/f.png}
\end{minipage}

\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/u_1.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/v_1.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/u+v_1.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/A(u+v)_1.png}
\end{minipage}


\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/u_8.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/v_8.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/u+v_8.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/A(u+v)_8.png}
\end{minipage}

\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/u_16.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/v_16.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/u+v_16.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/A(u+v)_16.png}
\end{minipage}

\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/u_50.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/v_50.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/u+v_50.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Morozov/rat = 0.001/A(u+v)_50.png}
\end{minipage}


\caption{Nested Bregman iteration with Morozov regularization (Algorithm \ref{algo:NestedBregman_Noisy_Morozov}) with $g(u) = \frac{1}{2}\norm{\nabla u}_{L^2}^2 $ and $ \beta h(v)= \beta \tv{v}$ for the weighting choice $\beta = 0.001$.\\
First line: true decomposition and observation.\\
Second line: Iterates for $l = 1$, PSNR =33.578 \\
Third line: Iterates for $l = 8$, PSNR = 34.3226\\
Fourth line: Iterates for $l = 16$, PSNR = 35.1054\\
Fifth line: Iterates for $l = 50$, PSNR = 32.678\\}

\label{fig:Nested_Morozov_ratio=0.001}

\end{figure}
%-------------------------------------------------now Bregman------------------------------

\begin{figure}[H]
    \centering
    \includegraphics[scale = 0.5]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/PSNR.png}
    \caption{PSNR values for the iterates obtained by Algorithm \ref{algo:NestedBregman_Noisy} with with $g(u) = \frac{\alpha}{2}\norm{\nabla u}_{L^2}^2 $ and $h(v)= \beta \tv{v}$ with weighting choice $\alpha = 465$, $\beta = 0.465$}
    \label{fig:Nested_Bregman_rat=0.001_PSNR}
\end{figure}

\begin{figure}[H]
\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/data/u.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/data/v.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/data/u+v.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/data/f.png}
\end{minipage}

\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/u_1.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/v_1.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/u+v_1.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/A(u+v)_1.png}
\end{minipage}


\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/u_8.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/v_8.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/u+v_8.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/A(u+v)_8.png}
\end{minipage}

\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/u_15.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/v_15.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/u+v_15.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/A(u+v)_15.png}
\end{minipage}

\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/u_50.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/v_50.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/u+v_50.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_H1_TV/Nested_Bregman/rat = 0.001/A(u+v)_50.png}
\end{minipage}




\caption{Nested Bregman iteration  (Algorithm \ref{algo:NestedBregman_Noisy}) with $g(u) = \frac{\alpha}{2}\norm{\nabla u}_{L^2}^2 $ and $ \beta h(v)=  \tv{v}$ for the weighting choice $\alpha =465 $, $\beta = 0.465$.\\
First line: true decomposition and observation.\\
Second line: Iterates for $l = 1$, PSNR = 34.5312 \\
Third line: Iterates for $l = 8$, PSNR = 34.9738\\
Fourth line: Iterates for $l = 15$, PSNR = 36.2136\\
Fifth line: Iterates for $l = 50$, PSNR = 33.272\\}

\label{fig:Nested_Bregman_ratio=0.001}

\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[scale = 0.5]{Images/Images_H1_TV/Comparison_Morozov_Nested.eps}
    \caption{Values of $h(v_l^\delta)$ in Algortihms \ref{algo:NestedBregman_Noisy_Morozov} and \ref{algo:NestedBregman_Noisy} vs the theoretical upper-bound from \eqref{eq:Convergence_h_noisy}.}
    \label{fig:nested_morozov_H1_TV_bound}
\end{figure}





% We derive the Chambolle-Pock algorithm to solve \begin{align*}
%  \min\limits_{\norm{A(u+v)-f}\le c} \frac{\alpha}{2}\norm{\nabla u}_{L^2}^2 + \tv{v} -\inner{p}{u}-\inner{q}{v} = \min\limits_{u,v}   \frac{\alpha}{2}\norm{\nabla u}_{L^2}^2 + \tv{v} -\inner{p}{u}-\inner{q}{v} +\I_{\norm{\cdot}\le c}(A(u+v)-f), \end{align*}
%  where $\norm{\cdot}$ denotes the Hilbert space norm on $Y = \ran A$. Approximating $\tv{v} \approx \norm{\nabla v}_{L^1}$ and discretizing, we obtain \begin{align*}
%      &\min\limits_{u,v}   \frac{\alpha}{2}\norm{\nabla u}_{2}^2 + \norm{\nabla v}_1 -\inner{p}{u}-\inner{q}{v} +\I_{\norm{\cdot}\le c}(A(u+v)-f) \\=& \min_{u,v}\max\limits_{y_1,y_2,y_3}  -\inner{p}{u}-\inner{q}{v} +\inner{y_1}{\nabla u} +\inner{y_2}{\nabla v} + \inner{y_3}{A(u+v)} -\pars{\frac{\norm{y_1}_2^2}{2\alpha} + \I_{\norm{\cdot }_\infty\le 1}(y_2) + c\norm{y_3}+\inner{y_3}{f}}.
%      \end{align*}
%      Therefore, we can apply the Chambolle-Pock algorithm with \begin{align*}
%          &K = \begin{pmatrix}
%            \nabla & 0\\
%            0 & \nabla \\
%            A&A
%          \end{pmatrix},
%          \\&G(u,v) = -\inner{p}{u} - \inner{q}{v}, 
%          \\&F^*(y_1,y_2,y_3) = \frac{\norm{y_1}_2^2}{2\alpha} + \I_{\norm{\cdot }_\infty\le 1}(y_2) + c\norm{y_3}+\inner{y_3}{f}.
%      \end{align*}
%      Note that \begin{align*}
%          &\argmin_{z} \frac{1}{2}\norm{y_3-z}^2 + c \norm{z} + \inner{z}{f} \\= &\argmin_z \frac{1}{2}\norm{y_3-(z-f)}^2 + c\norm{z} = \begin{cases}
%             0 &\text{ if } \norm{y_3-f} \le c\\
%             \pars{1-\frac{c}{\norm{y_3-f}}}(y_3-f) &\text{ else}
%          \end{cases},
%      \end{align*}
%      where $\norm{\cdot}$ denotes the Frobenius norm on $\ran A$.
%      This gives the following proximal operators\begin{align*}
%          &(Id + \tau \partial G)^{-1}(u,v) = (u+\tau p,v+\tau q)\\
%          &(Id + \sigma F^*)^{-1}(y_1,y_2,y_3) = \pars{\frac{y_1}{1+\frac{\sigma}{\alpha}},\frac{y_2}{\max\set{1,\abs{y_2}}},\squarebrackets{1-\frac{\sigma c}{\norm{y_3-\sigma f}}}_+(y_3-\sigma f)}.
%      \end{align*}
%      Hence, we reach the update scheme:\begin{align*}
%          y_1^{n+1} &= \frac{y1^n+\sigma \nabla \bar u^n}{1+\frac{\sigma}{\alpha}},\\
%          y_2^{n+1} &= \frac{y_2+\sigma \nabla \bar u^n}{\max\set{1,\abs{y_2+\sigma \nabla \bar v^n}}},\\
%          y_3^{n+1} &= \squarebrackets{1-\frac{\sigma c}{\norm{y_3^n+A(\bar u^n+\bar v^n)-\sigma f)}}}_+(y_3^n+A(\bar u^n+\bar v^n)-\sigma f), \\
%          u^{n+1} &= u^n+\tau \div( \nabla y_1^{n+1}) -\tau A^*y_3^{n+1} +\tau p,\\
%          v^{n+1} &= v^n+\tau \div (\nabla y_2^{n+1}) -\tau A^*y_3^{n+1} +\tau q,\\
%          \bar u^{n+1} &= 2u^{n+1}-u^n,\\
%          \bar v^{n+1} &= 2v^{n+1} -v^n.
%      \end{align*}
% In order to turn this into Nested Bregman iterations we update either $u^{n+1} = -\alpha \div (\nabla u^n)$ or $q^{n+1} = q^n -\alpha \div (\nabla u^n)$.\subsection{Oscillation TGV}
We conclude the numerical experiments by illustrating the method for more complicated functionals. For this we choose the infimal convolution of the total generalized variation and the oscillation TGV. As a test image, we consider the sum of a square with piecewise affine texture $u^*$ and an oscillating pattern with the space for the square being cut out $v^*$ (see line 1 in Figure \ref{fig:TGV_osci_Nested_Morozov}). The oscillations follow the definition \begin{equation*}
    \cos(\omega\cdot x) + \sin(\omega\cdot x)
\end{equation*} with $x \in \Omega = [0,N]^2$ for $(\omega_1,\omega_2) = (0.25,0.5)$ and $N = 75$ being the number of pixels of one of the $9$ sub-squares of the complete image. The observation $f^\delta$ was created by adding Gaussian noise (mean $0$ and variance $\sigma = 0.05$) to the sum $u^*+v^*$. We then ran Algorithm \ref{algo:NestedBregman_Noisy_Morozov} with $g(u) = TGV_{\alpha_1,\beta_1}(u)$ and $h(v) = TGV{osci}_{\alpha_2,\beta_2,c}(v)$ with $c = \omega \otimes \omega$. As initial guess for the parameters we consider $\alpha_1 = 5$ and $\alpha_2 = 1$. Following the numerical experiments used to obtain Figure 3 in \cite{oscICTV}, we choose $\beta_i = 2\alpha_i$ for $i = 1,2$. The results after $l = 1,2,10$ iterations can be seen in lines $2-4$ of Figure \ref{fig:TGV_osci_Nested_Morozov}. We note that after the first iteration, the component $u_1$ is over-regularized so that the share of the $v$ component to the overall reconstruction needs to be decreased. We therefore replace $g$ with suitable Bregman distances as suggested by Algorithm \ref{algo:NestedBregman_Noisy_Morozov}. This results in  a notable improvement of the decomposition after only $1$ additional iteration (line 3). As expected, eventually too much information of the $v$ component is contained in the $u$ component (line 10). This once again stresses the need for an appropriate stopping criterion for the iteration. \tw{I also observe that the PSNR decreases with the iteration. I am not entirely sure why this is. To be honest, I believe that the complicated calculation of the subdifferentials (see also the numerical derviation of the method later) results in the numerics being less statble than for the previuous exapmles. But it could also be due to the choice of components and regularizers.} 




\begin{figure}[H]
\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/u_true.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/v_true.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/x_true.png}
\end{minipage}

\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/u_1.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/v_1.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/x_1.png}
\end{minipage}

\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/u_2.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/v_2.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/x_2.png}
\end{minipage}


\centering
\hspace{-4cm}\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/u_10.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/v_10.png}
\end{minipage}\hspace{3cm}
\begin{minipage}[c]{0.1\textwidth}
    \includegraphics[scale = 0.4]{Images/Images_osci/Nested/x_10.png}
\end{minipage}




    \caption{Nested Bregman iteration (Algorithm \ref{algo:NestedBregman_Noisy_Morozov}) for $g(u) = TGV_{\alpha_1,\beta_1}(u)$ and $h(v) = TGV^{osci}_{\alpha_2,\beta_2,c}$ for the weighting choice $\alpha_1 = 5$, $\alpha_2 = 1$ and $\beta_i = 2\alpha_i$ for $i = 1,2$. \\
    First line: true decomposition and observation\\
    Second line: Iterates for $l =1$, PSNR= 35.5047\\
    Third line: Iterates for $l = 2$, PSNR =30.5265\\
    Fourth line: Iterates for $l = 10$, PSNR = 26.497}
    \label{fig:TGV_osci_Nested_Morozov}
\end{figure}
